Invariant Flags for Singularly Perturbed Logarithmic Systems of Rank Two

We study rank-two differential systems $\hbar x \partial_x \psi + A (x, \hbar) \psi = 0$ near a logarithmic pole, with coefficients that are holomorphic in $x$ and admit uniform factorial asymptotic expansions in the complex parameter $\hbar$. If the classical residue has distinct eigenvalues, then upon choosing an ordering and an admissible $\hbar$ direction, we transform this system to an upper-triangular form by a holomorphic gauge transformation with the same factorial asymptotic regularity on a sector in the $\hbar$-plane. Its diagonal is fully determined by the $\hbar \to 0$ and $x \to 0$ limits. This construction produces a canonical $(x,\hbar)$-dependent invariant flag. This flag specialises to the usual Levelt filtration for nonzero values of $\hbar$ on a narrower sector, and its associated graded converges to the eigenspaces of the residue as $x \to 0$ and of the leading-order matrix as $\hbar \to 0$. A Schr\"odinger example gives a uniform matching formula between the WKB data and the exact Frobenius exponent at a double pole.

==> src/project-preamble.tex <==
% Load this project's frozen house packages rather than globally installed copies.
% File substitution also covers dependencies requested internally by other packages.
\makeatletter
\declare@file@substitution{declare-style.sty}{src/declare-style.sty}
\declare@file@substitution{declare-style-notes.sty}{src/declare-style-notes.sty}
\declare@file@substitution{declare-maths.sty}{src/declare-maths.sty}
\declare@file@substitution{declare-text.sty}{src/declare-text.sty}
\declare@file@substitution{declare-tables-figures.sty}{src/declare-tables-figures.sty}
\declare@file@substitution{declare-theorems-notes.sty}{src/declare-theorems-notes.sty}
\declare@file@substitution{declare-bibliography.sty}{src/declare-bibliography.sty}
\makeatother

